Accuracy, Estimates, and Representation Results

Measures of accuracy usually score how accurate a specified credence depending on whether the proposition is true or false. A key requirement for such measures is strict propriety; that probabilities expect themselves to be most accurate. We discuss characterisation results for strictly proper measures of accuracy. By making some restrictive assumptions, we present the proof of the characterisation result of Schervish (1989) in an accessible way. We will also present the characterisation in terms of Bregman divergences and the relationship between the two characterisations. The new contribution of the paper is to show that the Schervish form characterises proper measures of accuracy for estimates of random variables more generally, by offering a converse to Schervish, Seidenfeld, and Kadane (2014, Lemma 1). We also provide a Bregman divergence characterisation in the estimates setting, using the close relationship between the two forms.

==> commands-2.tex <==

\makeatletter

\NeedsTeXFormat{LaTeX2e}

\raggedbottom


\newcommand*{\acknowledgement}[1]{\gdef\@acknowledgement{#1}}
\newcommand*{\@acknowledgement}{}
\renewcommand*{\@author}{\tobeblinded[Omitted for review]{Catrin Campbell-Moore\footnote{\@acknowledgement}}}


\newcommand{\tobeblinded}[2][OMITTED]{#2} %
\newcommand{\blindversion}{
\renewcommand{\tobeblinded}[2][OMITTED]{##1} %
}

		

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathrsfs} %
\usepackage{mathtools}

\usepackage{centernot}
\usepackage[usenames,dvipsnames,table]{xcolor}
\usepackage{wasysym}
\usepackage{xspace}	

\usepackage{stmaryrd}
\usepackage{thmtools}
\usepackage{units}

\usepackage{tikz}
\usetikzlibrary{positioning,calc,decorations.pathreplacing,decorations.markings,intersections,fit,patterns,shapes,arrows.meta,
}
\usepackage{pgfplots}
\usepackage{eso-pic,picture}
\usepackage{graphicx}




\usepackage{eurosym}
\usepackage{tabularx}
\usepackage{etoolbox} %
\usepackage{xparse}
\usepackage{multirow}
\usepackage{changepage} 
\usepackage{bm}
\usepackage{microtype} %
\usepackage{booktabs}
\usepackage{enumitem} %
\usepackage[textsize=footnotesize,obeyFinal,backgroundcolor=white,bordercolor=gray!20,linecolor=gray!20]{todonotes} %



\usepackage[breaklinks,colorlinks,linkcolor=black,citecolor=black,urlcolor=gray,hypertexnames=false]{hyperref} %
\usepackage{cleveref} %





\usepackage[round,comma]{natbib}
\newcommand{\bibcommand}{
	\setlength{\bibsep}{.2pt}
	
\bibliography{/Users/cc15682/Dropbox/research/projects/mybib}
	\bibliographystyle{plainnat}
	\appendix
}





\allowdisplaybreaks[1]















\tikzset{every picture/.append style={font=\small}, every label/.style={align=center}, every node/.style={align=center}}
\pgfplotsset{compat=1.15}



\newcommand{\todoimportant}[2][]{}






\newcommand*{\draftversionprintonleft}[1]{%
	\gdef\@draftversionprintonleft{#1}%
}


\newcommand*{\draftversionprintonright}[1]{%
	\gdef\@draftversionprintonright{#1}%
}


\newcommand*{\@draftversionprintonleft}{
	Please check for updates
	\ifx\@draftversionprintonleft@url\@nnil
	\else
		\href{\@draftversionprintonleft@url}{here} or %
	\fi
	by \href{mailto:catrin.campbell-moore@bristol.ac.uk}{emailing me}
	}


\newcommand*{\@draftversionprintonright}{{\Huge Draft} \; \today}


		\newcommand{\draftversion}[1][\@nil]{%
			\gdef\@draftversionprintonleft@url{#1}%
			\AddToShipoutPicture{%
				\setlength{\@tempdimb}{.5\paperwidth}%
				\setlength{\@tempdimc}{.5\paperheight}%
				\setlength{\unitlength}{1pt}%
				\protect{\put(\strip@pt\@tempdimb,\strip@pt\@tempdimc){%
					\makebox(-515,0){\rotatebox{90}{ %
						\textcolor[gray]{0.6}{
							\@draftversionprintonleft
						}
					}}
					\makebox(515,0){\rotatebox{270}{
						\textcolor[gray]{0.6}{
							\@draftversionprintonright		%
						}
					}}
				}}
			}
		}	

		


	\newcommand{\latedraftversion}[1][\@nil]{
		\draftversionprintonleft{
			\ifx\@draftversionprintonleft@url\@nil
			\else
				Check for updates \href{\@draftversionprintonleft@url}{here} %
			\fi
		}
		\draftversion[#1]
	}	

	
	\newcommand{\preprint}[1][\@nil]{
	\draftversionprintonleft{Preprint}
	\draftversionprintonright{}
	\draftversion[#1]
}	






\newcommand{\deprecateddraft}{%
	\AddToShipoutPicture{%
		\setlength{\@tempdimb}{.5\paperwidth}%
		\setlength{\@tempdimc}{.5\paperheight}%
		\setlength{\unitlength}{1pt}%
		\protect{\put(\strip@pt\@tempdimb,\strip@pt\@tempdimc){%
			\makebox(-515,0){\rotatebox{90}{ %
				\textcolor[gray]{0.6}{
				\Huge	Deprecated version
				}
			}}
		}}
	}
}	





\newcommand{\envsign}{$\triangle$}

	
	\theoremstyle{plain} \newtheorem{theorem}{Theorem}[section]
	\theoremstyle{plain} \newtheorem{desired theorem}[theorem]{Desired Theorem}
	
	\theoremstyle{definition} \newtheorem{definitionx}[theorem]{Definition}
		\newenvironment{definition}
		  {\pushQED{\qed}\renewcommand{\qedsymbol}{\envsign}\definitionx}
		  {\popQED\enddefinitionx}	
	
	
	\theoremstyle{definition} \newtheorem{assumption}{Assumption}\crefname{assumption}{assumption}{assumptions}
	\theoremstyle{plain} \newtheorem{lemma}[theorem]{Lemma}
	\theoremstyle{plain} \newtheorem{sublemma}{Sublemma}[theorem]
	\theoremstyle{plain} \newtheorem{corollary}[theorem]{Corollary}
	\theoremstyle{plain} \newtheorem{proposition}[theorem]{Proposition}
	\theoremstyle{plain} \newtheorem{conjecture}[theorem]{Conjecture}
	\theoremstyle{plain} \newtheorem{criteria}{Criteria}
	
	
	


					

	\theoremstyle{remark}\newtheorem*{proofattemptx}{Proof Attempt}
	\newenvironment{proof attempt}
	  {\pushQED{\qed}\renewcommand{\qedsymbol}{\envsign}\proofattemptx}
	  {\popQED\endproofattemptx}
	  
	\theoremstyle{remark}\newtheorem*{proofideax}{Proof Idea}
	\newenvironment{proof idea}
	  {\pushQED{\qed}\renewcommand{\qedsymbol}{\envsign}\proofideax}
	  {\popQED\endproofideax}

	  
\newenvironment{proof sketch}{%
  \renewcommand{\proofname}{Proof Sketch}\proof}{\endproof}
  
	\theoremstyle{definition}\newtheorem{remarkx}[theorem]{Remark}
	\newenvironment{remark}
	  {\pushQED{\qed}\renewcommand{\qedsymbol}{\envsign}\remarkx}
	  {\popQED\endremarkx}
	  
	\theoremstyle{remark}\newtheorem*{answer}{Answer}
	\theoremstyle{definition} \newtheorem*{nb}{Note}
	\theoremstyle{plain}\newtheorem{claim}[theorem]{Claim}
	\theoremstyle{plain}\newtheorem{question}[theorem]{Question}
	\theoremstyle{definition} \newtheorem{notation}[theorem]{Notation}
	
	
	\theoremstyle{definition} \newtheorem{examplex}[theorem]{Example}
	\newenvironment{example}
	  {\pushQED{\qed}\renewcommand{\qedsymbol}{\envsign}\examplex}
	  {\popQED\endexamplex}	
	
	
	
	\theoremstyle{definition} \newtheorem{argument}[theorem]{Argument}
	\newtheorem{subtheorem}{Sub-Theorem}[theorem] 
	
	
	\theoremstyle{definition}\newtheorem{setupx}[theorem]{Setup}\newtheorem*{setupx*}{Setup}
	\newenvironment{setup}
	  {\pushQED{\qed}\renewcommand{\qedsymbol}{\envsign}\setupx}
	  {\popQED\endsetupx}	
	
	
	\newenvironment{principle}{\begin{description}[style=nextline]\item}{\end{description}}
	\newenvironment{highlighted}{\begin{description}[style=nextline]\item}{\end{description}}


	\newenvironment{inlinequote}{``}{''}


	
	


	



\newcommand\Tstrut{\rule{0ex}{2.6ex}}         %
\newcommand\Bstrut{\rule[-0.9ex]{0ex}{0ex}}   %














	\renewcommand{\phi}{\varphi}
	\renewcommand{\emptyset}{\varnothing}
	\renewcommand{\leq}{\leqslant}
	\renewcommand{\geq}{\geqslant}


	\newcommand{\enmath}[1]{\ensuremath{#1}\xspace}
	\newcommand{\ul}{\underline}
	\newcommand{\bb}{\mathbb}
	\newcommand{\mf}{\mathfrak}
	\newcommand{\fk}{\mathfrak}
	\newcommand{\noteq}{\neq}
	\newcommand{\comment}[1]{{\leavevmode\color{red}{#1}}}
	


	\newcommand{\liff}{\leftrightarrow}
	\newcommand{\lif}{\rightarrow}

	\newcommand{\N}{\bb{N}}
	\newcommand{\Q}{\bb{Q}}
	\newcommand{\powerset}[1]{\wp(#1)}
	\newcommand{\R}{\bb{R}}
	\renewcommand{\Re}{\mathbb{R}}
	\newcommand{\integers}{\bb{Z}}
	\newcommand{\convto}{\longrightarrow}
	\newcommand{\convupto}{\nearrow}
	\newcommand{\convdownto}{\searrow}
	\newcommand{\geqc}{\succeq}
	\newcommand{\gc}{\succ}
	\newcommand{\leqc}{\preceq}
	\newcommand{\lc}{\prec}
	\newcommand*\diff{\mathop{}\!\mathrm{d}} %
	\usepackage{physics}

	
	\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}
	\newcommand{\entails}{\vDash}
	\newcommand{\restricted}[1]{\!\upharpoonright_{#1}}
	\newcommand\SetSymbol[1][]{\nonscript\:#1\vert\nonscript\:
		\mathopen{}\allowbreak}
			\providecommand{\given}{\SetSymbol}
	\DeclarePairedDelimiterX\set[1]\{\}{%
		\renewcommand\given{\SetSymbol[\delimsize]}
		#1
	}
				\providecommand\cond{}
		\newcommand\CondProbSymbol[1][]{\nonscript\:#1\vert\nonscript\:
			\mathopen{}\allowbreak}
		\DeclarePairedDelimiterX\pr[1](){%
			\renewcommand\cond{\CondProbSymbol[\delimsize]}
			#1
		}
		
			\providecommand\updatecond{}
			\newcommand\updateProbSymbol[1][]{\nonscript\:#1\vert\vert\nonscript\:
				\mathopen{}\allowbreak}
			\DeclarePairedDelimiterX\updatepr[1](){%
				\renewcommand\updatecond{\updateProbSymbol[\delimsize]}
				#1
			}

	\DeclarePairedDelimiter\ordpair{\langle}{\rangle}
		\DeclarePairedDelimiter\ordseq{\langle}{\rangle}
	\DeclarePairedDelimiter\seq{\langle}{\rangle}
	
	
	\DeclarePairedDelimiter\modelsof{[}{]}%
	\DeclarePairedDelimiter\br{(}{)}
	\DeclarePairedDelimiter\squarebraces{[}{]}
	\newcommand{\invisbr}[1]{#1}
	
	
	\newcommand{\true}{\enmath{\sf{true}}}
	\newcommand{\false}{\enmath{\sf{false}}}
	\newcommand{\neither}{\enmath{\sf{neither}}}
	\newcommand{\ahalf}{\enmath{\nicefrac{1}{2}}}


		\newcommand{\curlyl}{\prec}
		\newcommand{\curlyleq}{\preceq}
		\newcommand{\curlygeq}{\succeq}
		\newcommand{\curlyg}{\succ}
		\newcommand{\curlyeq}{\approx}
		
	\DeclareMathOperator*{\argmin}{arg\,min}

\newbox\gnBoxA
\newdimen\gnCornerHgt
\setbox\gnBoxA=\hbox{$\ulcorner$}
\global\gnCornerHgt=\ht\gnBoxA
\newdimen\gnArgHgt

\newcommand{\gnraised}[1]{
	\setbox\gnBoxA=\hbox{$#1$}%
	\gnArgHgt=\ht\gnBoxA%
	\ifnum \gnArgHgt<\gnCornerHgt
	\gnArgHgt=0pt%
	\else
	\advance \gnArgHgt by -\gnCornerHgt%
	\fi
	\raise\gnArgHgt\hbox{$\ulcorner$} \box\gnBoxA %
	\raise\gnArgHgt\hbox{$\urcorner$}
}


\NewDocumentCommand\gn{sm}{%
	\IfBooleanTF{#1}%
	{\gnraised{#2}}%
	{\ulcorner #2 \urcorner}%
}



	\newcommand{\subdot}[1]{\oalign{$#1$\cr\hfil.\hfil}}
	\newcommand{\supdot}[1]{\dot{#1}}
	\renewcommand{\bar}[1]{\overline{#1}}






\DeclareDocumentCommand \enumsentence { o m } {%
	\IfNoValueTF {#1} {%
		\begin{equation*}
						\text{\parbox{.85\textwidth}{#2}}
					\end{equation*}
	}{%
	\leqnomode
	\begin{align}\tag{#1}
					\qquad&\text{\parbox{.85\textwidth}{#2}}
				\end{align}
	\reqnomode
}%
}


	\newcommand{\mathquote}[1]{\text{`}\,#1\,\text{'}}
	\newcommand{\defemph}[1]{\emph{#1}\index{#1}}
	
	
	
	\newcommand{\prop}[1]{\textsc{#1}\xspace}
	\newcommand{\heads}{\prop{Heads}}
	\newcommand{\tails}{\prop{Tails}}
	\newcommand{\Yellow}{\prop{Yellow}}
	\newcommand{\Blue}{\prop{Blue}}
	\newcommand{\Red}{\prop{Red}}

	
	\newcommand{\Sent}[1][]{{\sf{Sent}_{{#1}}}}
	\newcommand{\Sat}{\sf{Sat}}
	\renewcommand{\Form}[1][]{\sf{Form}_{{#1}}}
	\newcommand{\rk}{\sf{rk}}
	\newcommand{\PA}{\sf{PA}}
	\newcommand{\Succ}{\sf{S}}
	
	\newcommand{\cartesianproduct}{\times}

	\newcommand{\On}{\sf{On}}


	\newcommand{\Nats}{N}
	\newcommand{\Reals}{R}
	\newcommand{\Probs}{\sf{Probs}}
	
	
	\newcommand{\lang}{\cal{L}}
	


\newcommand{\propvar}{\prop{O}}


\newcommand{\T}{T}
\newcommand{\Cr}{C\hspace*{-1pt}r}



\newcommand{\mT}{\mathrm{T}}


\newcommand{\samplespace}{\Omega}
\newcommand{\Worlds}{W}
\newcommand{\world}{w}
\newcommand{\measalg}{\cal{F}}

\newcommand{\meas}{m}

\newcommand{\lowerprob}{\underline{\mP}}
\newcommand{\upperprob}{\overline{\mP}}

\newcommand{\chance}{\sf{ch}}
\newcommand{\mchance}{\mathrm{ch}}


		
	\newcommand{\liar}{\enmath{\mathtt{Liar}}}
	\newcommand{\detliar}{\enmath{\mathtt{DetLiar}}}
	\newcommand{\truthteller}{\enmath{\mathtt{TruthTeller}}}
	\newcommand{\mcgee}{\enmath{\mathtt{McGee}}}
	\newcommand{\prliar}{\enmath{\mathtt{CredLiar}}}
	
	
	\newcommand{\leap}{\prop{Leap}}
	\newcommand{\rain}{\prop{Rain}}
	\newcommand{\passport}{\prop{Passport}}
	\newcommand{\promotion}{\prop{Promotion}}
	\newcommand{\badnavigator}{\prop{BadNavigator}}







\newcommand{\rev}{\rho}



\newcommand{\brierscore}{\sf{BS}}
\newcommand{\logscore}{\sf{LS}}
\newcommand{\Acc}{\mathsf{Acc}}
\newcommand{\acc}{\mathsf{acc}}



\newcommand{\money}[1]{\text{\pounds} {#1}}
\newcommand{\pence}{p\xspace}






\newcommand{\Est}{\mathrm{Est}}
\newcommand{\Exp}{\mathrm{Exp}}

\newcommand{\IP}[1][P]{{\mathbb{#1}}}
\newcommand{\IPB}{{\IP[B]}}
\newcommand{\IPC}{{\IP[C]}}
\newcommand{\rec}{\mathsf{rec}}

\newcommand{\Value}{\mathsf{Value}}

\newcommand{\iprec}{{Imprecise Recommendation}\xspace}





\newcommand{\Creds}{\mathsf{Creds}}


\usepackage{versions}
\newcommand{\deleteallfollowing}{\newpage\leavevmode\color{blue} \begin{center}
{\huge \bfseries Delete Everything from Here Onwards}
\end{center}}
\newenvironment{tobedeleted}{\leavevmode\color{red} }{}
\newenvironment{suggestion}{\leavevmode\color{blue}}{}
\newenvironment{note}{\leavevmode\color{blue}}{}




\usepackage{pifont}%
\newcommand{\cmark}{\text{\ding{51}}}%
\newcommand{\xmark}{\text{\ding{55}}}%




	








\renewcommand{\false}{\nottrue}
\newcommand{\nottrue}{{\textsf{not-true}}\xspace}




\newcommand{\pause}{}



\tikzset{				
	point/.style={fill=black,circle,inner sep=1pt},
	arrow/.style={-{Latex[width=1mm]},shorten <=2pt,shorten >=2pt},
}


\newcommand{\closure}{\mathsf{closure}}		








\makeatother

